The Role of Local Intrinsic Dimensionality in Benchmarking Nearest Neighbor Search

This paper reconsiders common benchmarking approaches to nearest neighbor search. It is shown that the concept of local intrinsic dimensionality (LID) allows to choose query sets of a wide range of difficulty for real-world datasets. Moreover, the effect of different LID distributions on the running time performance of implementations is empirically studied. To this end, different visualization concepts are introduced that allow to get a more fine-grained overview of the inner workings of nearest neighbor search principles. The paper closes with remarks about the diversity of datasets commonly used for nearest neighbor search benchmarking. It is shown that such real-world datasets are not diverse: results on a single dataset predict results on all other datasets well.

==> __latexindent_temp.tex <==
@ARTICLE{Iwasaki18,
   author = {{Iwasaki}, M. and {Miyazaki}, D.},
    title = "{Optimization of Indexing Based on k-Nearest Neighbor Graph for Proximity Search in High-dimensional Data}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1810.07355},
 primaryClass = "cs.DB",
 keywords = {Computer Science - Databases, Computer Science - Information Retrieval},
     year = 2018,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv181007355I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{Houle13,
  title={Dimensionality, discriminability, density and distance distributions},
  author={Houle, Michael E},
  booktitle={Data Mining Workshops (ICDMW)},
  pages={468--473},
  year={2013},
  organization={IEEE}
}

@misc{annoy,
title = {Annoy},
author = {Erik Bernhardsson},
url = {https://github.com/spotify/annoy}
}

@article{faiss,
  author    = {Jeff Johnson and
               Matthijs Douze and
               Herv{\'{e}} J{\'{e}}gou},
  title     = {Billion-scale similarity search with GPUs},
  journal   = {CoRR},
  volume    = {abs/1702.08734},
  year      = {2017},
  misc      = {\url{https://github.com/facebookresearch/faiss}},
  timestamp = {Wed, 01 Mar 2017 14:26:00 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JohnsonDJ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{KriegelSZ17,
  author    = {Hans{-}Peter Kriegel and
               Erich Schubert and
               Arthur Zimek},
  title     = {The (black) art of runtime evaluation: Are we comparing algorithms
               or implementations?},
  journal   = {Knowl. Inf. Syst.},
  volume    = {52},
  number    = {2},
  pages     = {341--378},
  year      = {2017},
  timestamp = {Tue, 11 Jul 2017 18:48:57 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/kais/KriegelSZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{pennington2014glove,
  author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
  title = {GloVe: Global Vectors for Word Representation},
  year = {2014},
  pages = {1532--1543},
}

@inproceedings{HouleSZ18,
  author    = {Michael E. Houle and
               Erich Schubert and
               Arthur Zimek},
  title     = {On the Correlation Between Local Intrinsic Dimensionality and Outlierness},
  booktitle = {{SISAP}'18},
  pages     = {177--191},
  year      = {2018},
  doi       = {10.1007/978-3-030-02224-2\_14},
  timestamp = {Sat, 24 Nov 2018 11:59:43 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/sisap/HouleSZ18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{Falconer04,
  title={Fractal geometry: mathematical foundations and applications},
  author={Falconer, Kenneth},
  year={2004},
  publisher={John Wiley \& Sons}
}

@article{mlpack2013,
  title     = {{MLPACK}: A Scalable {C++} Machine Learning Library},
  author    = {Curtin, Ryan R. and Cline, James R. and Slagle, Neil P. and
               March, William B. and Ram, P. and Mehta, Nishant A. and Gray,
               Alexander G.},
  journal   = {J. of Machine Learning Research},
  volume    = {14},
  pages     = {801--805},
  year      = {2013}
}

@inproceedings{edel2014automatic,
      title={An automatic benchmarking system},
      author={Edel, Marcus and Soni, Anand and Curtin, Ryan R},
      year={2014},
      booktitle = {NIPS 2014 Workshop on Software Engineering for Machine Learning}
}

@article{LiZSWZL16,
  author    = {Wen Li and
               Ying Zhang and
               Yifang Sun and
               Wei Wang and
               Wenjie Zhang and
               Xuemin Lin},
  title     = {Approximate Nearest Neighbor Search on High Dimensional Data - Experiments,
               Analyses, and Improvement (v1.0)},
  journal   = {CoRR},
  volume    = {abs/1610.02455},
  year      = {2016},
  timestamp = {Wed, 07 Jun 2017 14:41:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiZSWZL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{JohnsonL86,
  title={{Extensions of Lipschitz maps into Banach spaces}},
  author={Johnson, William B and Lindenstrauss, Joram and Schechtman, Gideon},
  journal={Israel Journal of Mathematics},
  volume={54},
  number={2},
  pages={129--138},
  year={1986},
}

@inproceedings{Anshu17,
 author = {Spring, Ryan and Shrivastava, Anshumali},
 title = {Scalable and Sustainable Deep Learning via Randomized Hashing},
 booktitle = {{KDD}'17},
 year = {2017},
 isbn = {978-1-4503-4887-4},
 pages = {445--454},
 numpages = {10},
 doi = {10.1145/3097983.3098035},
 acmid = {3098035},
 keywords = {deep learning, locality-sensitive hashing, neural networks, parallel computing, randomized algorithms},
}

@article{word2vec,
  author    = {Tomas Mikolov and
               Kai Chen and
               Greg Corrado and
               Jeffrey Dean},
  title     = {Efficient Estimation of Word Representations in Vector Space},
  journal   = {CoRR},
  volume    = {abs/1301.3781},
  year      = {2013},
  archivePrefix = {arXiv},
  eprint    = {1301.3781},
  timestamp = {Mon, 13 Aug 2018 16:48:33 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1301-3781},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{fashion-mnist,
  author    = {Han Xiao and
               Kashif Rasul and
               Roland Vollgraf},
  title     = {Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning
               Algorithms},
  journal   = {CoRR},
  volume    = {abs/1708.07747},
  year      = {2017},
  archivePrefix = {arXiv},
  eprint    = {1708.07747},
  timestamp = {Mon, 13 Aug 2018 16:47:27 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1708-07747},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{JegouDS11,
  author    = {Herv{\'{e}} J{\'{e}}gou and
               Matthijs Douze and
               Cordelia Schmid},
  title     = {Product Quantization for Nearest Neighbor Search},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {33},
  number    = {1},
  pages     = {117--128},
  year      = {2011},
  doi       = {10.1109/TPAMI.2010.57},
  timestamp = {Wed, 14 Nov 2018 10:51:14 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/pami/JegouDS11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{hnsw,
   author = {{Malkov}, Y.~A. and {Yashunin}, D.~A.},
    title = "{Efficient and robust approximate nearest neighbor search using Hierarchical Navigable Small World graphs}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.09320},
 primaryClass = "cs.DS",
 keywords = {Computer Science - Data Structures and Algorithms, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Information Retrieval, Computer Science - Social and Information Networks},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160309320M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{ngt,
    author = {Yahoo Japan Corporation},
	title = {{NGT: PANNG}},
    url = {https://github.com/yahoojapan/NGT}
}

@inproceedings{nmslib,
  author    = {Leonid Boytsov and
               Bilegsaikhan Naidan},
  title     = {Engineering Efficient and Effective Non-metric Space Library},
  booktitle = {{SISAP}'13},
  pages     = {280--293},
  timestamp = {Mon, 02 Sep 2013 10:13:50 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/sisap/BoytsovN13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{amsaleg2019intrinsic,
  title={Intrinsic Dimensionality Estimation within Tight Localities},
  author={Amsaleg, Laurent and Chelly, Oussama and Houle, Michael E and Kawarabayashi, Ken-ichi and Radovanovi{\'c}, Milo{\v{s}} and Treeratanajaru, Weeris},
  booktitle={Proceedings of the 2019 SIAM International Conference on Data Mining},
  pages={181--189},
  year={2019},
  organization={SIAM}
}

@article{smithmiles14,
title = "Towards objective measures of algorithm performance across instance space",
journal = "Computers \& Operations Research",
volume = "45",
pages = "12 - 24",
year = "2014",
issn = "0305-0548",
doi = "https://doi.org/10.1016/j.cor.2013.11.015",
url = "http://www.sciencedirect.com/science/article/pii/S0305054813003389",
author = "Kate Smith-Miles and Davaatseren Baatar and Brendan Wreford and Rhyd Lewis",
}

@inproceedings{Amsaleg15,
  title={Estimating local intrinsic dimensionality},
  author={Amsaleg, Laurent and Chelly, Oussama and Furon, Teddy and Girard, Stephane and Houle, Michael E and Kawarabayashi, Ken-Ichi and Nett, Michael},
  booktitle={{KDD}'15},
  pages={29--38},
  year={2015},
  organization={ACM}
}

@inproceedings{AumullerBF17,
  author    = {Martin Aum{\"{u}}ller and
               Erik Bernhardsson and
               Alexander Faithfull},
  title     = {{ANN-Benchmarks: {A} Benchmarking Tool for Approximate Nearest Neighbor
               Algorithms}},
  booktitle = {{SISAP}'17},
  pages     = {34--49},
  year      = {2017},
  doi       = {10.1007/978-3-319-68474-1\_3},
  notes     = {Extended Version available at \url{https://arxiv.org/abs/1807.05614}},
  timestamp = {Wed, 14 Nov 2018 10:58:00 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/sisap/AumullerBF17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{AlmanW15,
   author    = {Josh Alman and
                Ryan Williams},
   title     = {Probabilistic Polynomials and Hamming Nearest Neighbors},
   booktitle = {FOCS'15},
   pages     = {136--150},
   timestamp = {Mon, 04 Jan 2016 13:44:40 +0100},
   biburl    = {http://dblp.uni-trier.de/rec/bib/conf/focs/AlmanW15},
   bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Williams05,
   author    = {Ryan Williams},
   title     = {A new algorithm for optimal 2-constraint satisfaction and its implications},
   journal   = {Theor. Comput. Sci.},
   volume    = {348},
   number    = {2-3},
   pages     = {357--365},
   year      = {2005},
   timestamp = {Tue, 18 Apr 2006 11:49:09 +0200},
   biburl    = {http://dblp.uni-trier.de/rec/bib/journals/tcs/Williams05},
   bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Levina05,
  title={Maximum likelihood estimation of intrinsic dimension},
  author={Levina, Elizaveta and Bickel, Peter J},
  booktitle={{NIPS}'15},
  pages={777--784},
  year={2005}
}
@article{Chavez01,
 author = {Ch\'{a}vez, Edgar and Navarro, Gonzalo and Baeza-Yates, Ricardo and Marroqu\'{\i}n, Jos{\'e} Luis},
 title = {Searching in Metric Spaces},
 journal = {ACM Comput. Surv.},
 issue_date = {September 2001},
 volume = {33},
 number = {3},
 month = sep,
 year = {2001},
 issn = {0360-0300},
 pages = {273--321},
 numpages = {49},
 doi = {10.1145/502807.502808},
 acmid = {502808},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Curse of dimensionality, nearest neighbors, similarity searching, vector spaces},
}

